NetSentry: A Deep Learning Approach to Detecting Incipient Large-scale Network Attacks

Machine Learning (ML) techniques are increasingly adopted to tackle ever-evolving high-profile network attacks, including DDoS, botnet, and ransomware, due to their unique ability to extract complex patterns hidden in data streams. These approaches are however routinely validated with data collected in the same environment, and their performance degrades when deployed in different network topologies and/or applied on previously unseen traffic, as we uncover. This suggests malicious/benign behaviors are largely learned superficially and ML-based Network Intrusion Detection System (NIDS) need revisiting, to be effective in practice. In this paper we dive into the mechanics of large-scale network attacks, with a view to understanding how to use ML for Network Intrusion Detection (NID) in a principled way. We reveal that, although cyberattacks vary significantly in terms of payloads, vectors and targets, their early stages, which are critical to successful attack outcomes, share many similarities and exhibit important temporal correlations. Therefore, we treat NID as a time-sensitive task and propose NetSentry, perhaps the first of its kind NIDS that builds on Bidirectional Asymmetric LSTM (Bi-ALSTM), an original ensemble of sequential neural models, to detect network threats before they spread. We cross-evaluate NetSentry using two practical datasets, training on one and testing on the other, and demonstrate F1 score gains above 33% over the state-of-the-art, as well as up to 3 times higher rates of detecting attacks such as XSS and web bruteforce. Further, we put forward a novel data augmentation technique that boosts the generalization abilities of a broad range of supervised deep learning algorithms, leading to average F1 score gains above 35%.

==> refs.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname href\endcsname\relax
  \def\href#1#2{#2} \def\path#1{#1}\fi

\bibitem{botstat}
{Spamhaus Botnet Threat Update: Q1-2021},
  \url{https://www.spamhaus.org/news/article/809/spamhaus-botnet-threat-update-q1-2021}.

\bibitem{lossstat}
C.~Ventures, {Global Cybercrime Damages Predicted To Reach \$6 Trillion
  Annually By 2021},
  \url{https://cybersecurityventures.com/cybercrime-damages-6-trillion-by-2021/}
  (2020).

\bibitem{beforeyouknew}
L.~Bilge, T.~Dumitra\c{s}, Before we knew it: An empirical study of zero-day
  attacks in the real world, in: Proc. ACM CCS, 2012.

\bibitem{buczak2015survey}
A.~L. Buczak, E.~Guven, A survey of data mining and machine learning methods
  for cyber security intrusion detection, IEEE Communications Surveys \&
  Tutorials 18~(2) (2016) 1153--1176.

\bibitem{lin2018idsgan}
Z.~Lin, et~al., {IDSGAN: Generative adversarial networks for attack generation
  against intrusion detection}, arXiv:1809.02077 (2019).

\bibitem{xia2015learning}
Y.~Xia, et~al., Learning discriminative reconstructions for unsupervised
  outlier removal, in: Proc. IEEE ICCV, 2015.

\bibitem{mirsky2018kitsune}
Y.~Mirsky, et~al., Kitsune: an ensemble of autoencoders for online network
  intrusion detection, in: NDSS, 2018.

\bibitem{sommer2010}
R.~{Sommer}, V.~{Paxson}, Outside the closed world: On using machine learning
  for network intrusion detection, in: IEEE S\&P, 2010.

\bibitem{ba20}
{Cyberint Research}, {British Airways Flight to DDoS Lands with Cyber
  Turbulence},
  \url{https://blog.cyberint.com/british-airways-flight-to-ddos-lands-with-cyber-turbulence}
  (March 2020).

\bibitem{gu2007bothunter}
G.~Gu, et~al., Bothunter: Detecting malware infection through ids-driven dialog
  correlation., in: USENIX Security, 2007.

\bibitem{ifflander2019hands}
L.~Iffl{\"a}nder, et~al., Hands off my database: Ransomware detection in
  databases through dynamic analysis of query sequences, arXiv preprint
  arXiv:1907.06775 (2019).

\bibitem{antonakakis2017understanding}
M.~Antonakakis, et~al., {Understanding the Mirai botnet}, in: USENIX Security,
  2017.

\bibitem{hutchins2011intelligence}
E.~M. Hutchins, et~al., Intelligence-driven computer network defense informed
  by analysis of adversary campaigns and intrusion kill chains, Leading Issues
  in Information Warfare \& Security Research (2011).

\bibitem{owasp}
E.~Saad, et~al., {OWASP Web Security Testing Guide Version 4.1} (2019).

\bibitem{eternalblue}
C.~C. Vulnerabilities, Exposures, {CVE-2017-0144},
  \url{https://cve.mitre.org/cgi-bin/cvename.cgi?name=CVE-2017-0144} (Sept.
  2016).

\bibitem{kao2018dynamic}
D.-Y. Kao, S.-C. Hsiao, The dynamic analysis of wannacry ransomware, in: Proc.
  ICACT, 2018.

\bibitem{flowmeter}
C.~I. for Cybersecurity, {CICFLOWMETER},
  \url{https://www.unb.ca/cic/research/applications.html#CICFlowMeter} (2018).

\bibitem{ids2018}
T.~C.~S. Establishment, C.~I. for Cybersecurity, {A Realistic Cyber Defense
  Dataset (CSE-CIC-IDS2018)},
  \url{https://registry.opendata.aws/cse-cic-ids2018/} (2018).

\bibitem{hochreiter1997long}
S.~Hochreiter, J.~Schmidhuber, Long short-term memory, Neural computation 9~(8)
  (1997) 1735--1780.

\bibitem{sutskever2014sequence}
I.~Sutskever, O.~Vinyals, Q.~V. Le, Sequence to sequence learning
  with neural networks, Advances in neural information processing systems 27
  (2014).

\bibitem{kumar2022land}
S.~Kumar, D.~Kumar, P.~K. Donta, T.~Amgoth, Land subsidence
  prediction using recurrent neural networks, Stochastic Environmental Research
  and Risk Assessment 36~(2) (2022) 373--388.

\bibitem{xingjian2015convolutional}
S.~Xingjian, et~al., {Convolutional LSTM network: A machine learning approach
  for precipitation nowcasting}, in: NeurIPS, 2015.

\bibitem{he2016deep}
K.~He, X.~Zhang, S.~Ren, J.~Sun, Deep residual learning for image
  recognition, in: Proceedings of the IEEE conference on computer vision and
  pattern recognition, 2016, pp. 770--778.

\bibitem{yang2021msta}
J.~Yang, S.~Xiao, A.~Li, W.~Lu, X.~Gao, Y.~Li, Msta-net: Forgery
  detection by generating manipulation trace based on multi-scale self-texture
  attention, IEEE Transactions on Circuits and Systems for Video Technology
  (2021).

\bibitem{deepfp}
P.~Sirinam, et~al., Deep fingerprinting: Undermining website fingerprinting
  defenses with deep learning, in: Proc. ACM CCS, 2018.

\bibitem{zhang:2019}
C.~{Zhang}, et~al., Multi-service mobile traffic forecasting via convolutional
  long short-term memories, in: Proc. IEEE International Symposium on
  Measurements \& Networking, 2019.

\bibitem{jiang2020network}
K.~Jiang, et~al., Network intrusion detection combined hybrid sampling with
  deep hierarchical network, IEEE Access 8 (2020).

\bibitem{glorot2010understanding}
X.~Glorot, Y.~Bengio, Understanding the difficulty of training deep feedforward
  neural networks, in: Proc. AISTATS, 2010.

\bibitem{raghu2021vision}
M.~Raghu, T.~Unterthiner, S.~Kornblith, C.~Zhang, A.~Dosovitskiy,
  Do vision transformers see like convolutional neural networks?, Advances in
  Neural Information Processing Systems 34 (2021).

\bibitem{sharafaldin2018toward}
I.~Sharafaldin, et~al., Toward generating a new intrusion detection dataset and
  intrusion traffic characterization., in: ICISSP, 2018.

\bibitem{lee1998data}
W.~Lee, S.~Stolfo, Data mining approaches for intrusion detection, in: USENIX
  Security Symposium, 1998.

\bibitem{ruff2018deep}
L.~Ruff, et~al., Deep one-class classification, in: International
  conference on machine learning, 2018, pp. 4393--4402.

\bibitem{zong2018deep}
B.~Zong, Q.~Song, M.~R. Min, W.~Cheng, C.~Lumezanu, D.~Cho, H.~Chen, {Deep
  autoencoding Gaussian mixture model for unsupervised anomaly detection}, in:
  ICLR, 2018.

\bibitem{jetson}
NVIDIA, {Jetson Nano | NVIDIA Developer},
  \url{https://developer.nvidia.com/embedded/jetson-nano} (2019).

\bibitem{stinson2008towards}
E.~Stinson, J.~C. Mitchell, Towards systematic evaluation of the evadability of
  bot/botnet detection methods., WOOT 8 (2008).

\bibitem{co2019}
K.~T. Co, et~al., Procedural noise adversarial examples for black-box attacks
  on deep convolutional networks, in: ACM CCS, 2019.

\bibitem{zhang:2020}
C.~Zhang, et~al., Tiki-taka: Attacking and defending deep learning-based
  intrusion detection systems, in: ACM CCSW, 2020.

\bibitem{gu2008botsniffer}
G.~Gu, et~al., Botsniffer: Detecting botnet command and control channels in
  network traffic, in: Network and Distributed System Security Symposium
  (NDSS), 2008.

\bibitem{kolbitsch2009effective}
C.~Kolbitsch, et~al., Effective and efficient malware detection at the end
  host., in: USENIX Security Symposium, Vol.~4, 2009, pp. 351--366.

\bibitem{naderi2019malmax}
A.~Naderi-Afooshteh, et~al., Malmax: Multi-aspect execution for automated
  dynamic web server malware analysis, in: ACM CCS, 2019.

\bibitem{krupp2016identifying}
J.~Krupp, et~al., Identifying the scan and attack infrastructures behind
  amplification ddos attacks, in: Proc. ACM CCS, 2016.

\bibitem{yi2011incremental}
Y.~Yi, et~al., {Incremental SVM Based on Reserved Set for Network Intrusion
  Detection}, Expert Systems with Applications 38~(6) (2011) 7698--7707.

\bibitem{sangkatsanee2011practical}
P.~Sangkatsanee, et~al., Practical real-time intrusion detection using machine
  learning approaches, Computer Communications 34~(18) (2011) 2227--2235.

\bibitem{li2019mad}
D.~Li, D.~Chen, B.~Jin, L.~Shi, J.~Goh, S.-K. Ng, Mad-gan:
  Multivariate anomaly detection for time series data with generative
  adversarial networks, in: International Conference on Artificial Neural
  Networks, Springer, 2019, pp. 703--716.

\bibitem{du2019lifelong}
M.~Du, et~al., Lifelong anomaly detection through unlearning, in: Proc. ACM
  CCS, 2019.

\bibitem{shen2018tiresias}
Y.~Shen, et~al., Tiresias: Predicting security events through deep learning,
  in: Proc. ACM CCS, 2018.

\bibitem{su2019robust}
Y.~Su, Y.~Zhao, C.~Niu, R.~Liu, W.~Sun, D.~Pei, Robust anomaly detection for
  multivariate time series through stochastic recurrent neural network, in:
  Proc. ACM SIGKDD international conference on knowledge
  discovery \& data mining, 2019, pp. 2828--2837.

\bibitem{liu2020deep}
Y.~Liu, S.~Garg, J.~Nie, Y.~Zhang, Z.~Xiong, J.~Kang, M.~S. Hossain, Deep
  anomaly detection for time-series data in industrial iot: A
  communication-efficient on-device federated learning approach, IEEE Internet
  of Things Journal 8~(8) (2020) 6348--6358.

\bibitem{deng2021graph}
A.~Deng, B.~Hooi, Graph neural network-based anomaly detection in
  multivariate time series, in: AAAI, Vol.~35, 2021, pp. 4027--4035.

\bibitem{audibert2020usad}
J.~Audibert, P.~Michiardi, F.~Guyard, S.~Marti, M.~A. Zuluaga,
  USAD: unsupervised anomaly detection on multivariate time series, in:
  Proceedings of the 26th ACM SIGKDD International Conference on Knowledge
  Discovery \& Data Mining, 2020, pp. 3395--3404.

\bibitem{diro2018leveraging}
A.~Diro, N.~Chilamkurti, Leveraging lstm networks for attack detection in
  fog-to-things communications, IEEE Communications Magazine 56~(9) (2018)
  124--130.

\bibitem{li2018semantic}
Z.~Li, Z.~Qin, A semantic parsing based lstm model for intrusion detection, in:
  ICONIP, 2018.

\end{thebibliography}
